PatternPaint: Practical Layout Pattern Generation Using Diffusion-Based Inpainting

Generating diverse VLSI layout patterns is essential for various downstream tasks in design for manufacturing, as design rules continually evolve during the development of new technology nodes. However, existing training-based methods for layout pattern generation rely on large datasets. In practical scenarios, especially when developing a new technology node, obtaining such extensive layout data is challenging. Consequently, training models with large datasets becomes impractical, limiting the scalability and adaptability of prior approaches. To this end, we propose PatternPaint, a diffusion-based framework capable of generating legal patterns with limited design-rule-compliant training samples. PatternPaint simplifies complex layout pattern generation into a series of inpainting processes with a template-based denoising scheme. Furthermore, we perform few-shot finetuning on a pretrained image foundation model with only 20 design-rule-compliant samples. Experimental results show that using a sub-3nm technology node (Intel 18A), our model is the only one that can generate legal patterns in complex 2D metal interconnect design rule settings among all previous works and achieves a high diversity score. Additionally, our few-shot finetuning can boost the legality rate with 1.87X improvement compared to the original pretrained model. As a result, we demonstrate a production-ready approach for layout pattern generation in developing new technology nodes.

==> PatPaint/4.1_Experiment_EUV_7nm.tex <==
\section{Experiment: Uni-7nm}
\label{sec:uni-7}
In this experiment, we evaluate our solutions on a relatively simple Design Rules setting that only involves unidirectional wires, following the definition of \cite{Deepattern}. In this experiment, we will form rigorous comparisons with existing solutions, and quantitatively show that, at the pixel-level, the performance difference with existing solutions.


\input{PatPaint/tables/EUV-Comparison}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{PatPaint/figs/Unidirectional_7nm_Comparison.pdf}
    \vspace{-10pt}
    \caption{A Qualitative evaluation of the generated images for CUP \cite{CUP}, DiffPattern \cite{Diffpattern} as well as Ours work. DiffPattern-1k denoted the diffusion model trained on 1k images, DiffPattern-200 denoted diffusion model trained on 200 images, DiffPattern-20 denoted diffusion model trained on 20 images. Similarly, CUP-1000 \cite{CUP} is trained 1000 samples. In our settings, only PatternPaint is able to generate nearly noise-free image, Diffusion starts to produce legal images when the starter patterns(for training) are larger than 200.}
    \label{fig:EUV-qualitative}
\end{figure*}

\subsection{Experimental Setup}
\textbf{Uni-7nm} is a synthetic EUV 7nm unidirectional design rule setting following the similar definition of \cite{Deepattern}. For this unidirectional dataset, we will only check the E2E spacing as well as the minimum width of a given wire. In this unidirectional setting, all the vertical tracks are fixed so that only horizontal positions (minimum width and E2E) are being checked. We generate 1000 starter patterns with 128 x 128 pixels using a nonlinear solver.  Now, we predefined each delta-x and delta-y as 1 pixel, this image also becomes a topology matrix in squish representation and will be used as the training samples for CUP~\cite{CUP} and Diffpattern~\cite{Diffpattern}.

\textbf{PatternPaint model settings:} In this experiment, we employed a pre-trained model (stabldiffusion1.5-inpaint) for pattern generation, denoted as PatternPaint.
During inpainting, a mask that masked 1/8 region will be randomly generated and fed to the model, the model will perform inpainting within the masked region of a given starter sample and create new layout patterns. 

\textbf{Baseline methods:}
We compare our methods with a Variational Convolution Auto-encoder～\cite{VAE_autoencoder} (VCAE) based solution CUP~\cite{CUP} and diffusion-based solution Diffpattern~\cite{Diffpattern}. Our CUP VCAE and LegalGAN implementation follows the network configurations of \cite{CUP}. VCAE model is trained with 500 epochs with a learning rate of 0.0002. And LegalGAN model is trained with 200 epochs with a learning rate of 0.002.  We also follow the \cite{Diffpattern} to implement a diffusion-based solution. For each diffusion model, we train 400 epochs with a learning rate of 0.0001. 
% As for Diffpattern, since it is not open-sourced and there is very limited information online about the discrete diffusion model, we tried our best to implement a diffusion model on continuous space. While it has some discrepancies with Diffpattern, we argue that our diffusion-based implementation is still very powerful and managed to outperform the existing VCAE solutions as shown in later experiments. For each diffusion model, we train 400 epochs with a learning rate of 0.0001. 
%For LayouTransformer~\cite{LayouTransformer}, we did not choose to reimplement this method as transformer is known for requiring a large dataset to train. We don't think LayouTransformer will be able to learn the sequential modeling under this limited sample thus do not compare it here. 

\subsection{Comparison}
Table~\ref{tab:EUV_Comparison} presents the experiments comparing PatternPaint with baseline methods using training sample (starter pattern) sizes of 20, 200, and 1000. Given the prevalence of noise in pixel-based solutions, we quantitatively assessed the noise levels in the generated images. We defined noise pixels as those where three of its surrounding pixels (up, down, left, right) have opposite values. Noise level is defined as counting the percentage of noise pixels in a given image. 

\subsubsection{Noise Level Analysis}
Trained with 1000 starter patterns, CUP (VCAE) constantly produces noisy images with a Noise Level of 8\%. After performing LegalGAN, the noise level soon reduces to 0.5\%, however, the generated images still remain noisy as shown in CUP-1000 in Figure~\ref{fig:EUV-qualitative}. The DiffPattern method exhibits a significant reduction in noise as the number of training samples increases, dropping from 98.7\% to 0.44\%. PatternPaint achieves the lowest noise levels, registering just 0.03\% before implementing our template-based denoising scheme. This performance indicates PatternPaint’s potential to directly generate usable layout patterns at the pixel level.

% \subsubsection{Design Rule Checking}
% Diffusion-based solutions begin to yield DRC-compliant patterns with a minimum of 200 training samples. With 1000 samples, these methods successfully generate compliant patterns in about 25\% of cases. PatternPaint demonstrates superior performance by producing 820 legal patterns from 2000 generated images, benefiting from its remarkably low noise level. CUP (VCAE + LegalGAN) fails to produce any DRC-compliant patterns, due to the noise presence in the generated patterns.

% \subsubsection{Qualitative Evaluation}
% Figure~\ref{fig:EUV-qualitative} presents a qualitative comparison of layout patterns generated by PatternPaint and other baseline methods. DiffPattern-1k, DiffPattern-200, and DiffPattern-20 represent the diffusion models trained on 1000, 200, and 20 images, respectively. Similarly, CUP-1000 \cite{CUP} denotes a model trained on 1000 samples. Notably, PatternPaint consistently produces nearly noise-free images, highlighting its superior performance. In contrast, diffusion models only begin to produce legally compliant images when trained with more than 200 samples. The CUP-1000 (VCAE+LegalGAN) model struggles significantly, failing to accurately capture the skeleton of layout patterns. This results in noisy and non-rectangular polygon shapes being generated. fails to produce legal patterns at the pixel-level.


==> PatPaint/_backup_4_experimental_result.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.245\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/Unique Count.pdf}
    \caption{Unique Count}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/Entropy.pdf}
    \caption{Entropy $H_2$}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/Silhouette Score.pdf}
    \caption{Silhouette Score}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/Density.pdf}
    \caption{Density}
    \end{subfigure}
    \caption{Experiments results for iterative generation process, four metrics are examined: unique pattern counts, the density of generated images, silhouette\_score as well as Entropy ($H_2$)}
    \label{fig:iterative}
\end{figure*}
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/default_20_crop.pdf}
   % \caption{PCA plot for default-20 (sil\_score, high)}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/sd2_20_crop.pdf}
    % \caption{PCA plot for sd2-20, (sil\_score, low)}
    \end{subfigure}
    
    \caption{Interpretation of silhouette score using PCA 3D plot, left: default-20 (sil\_score, high), right:sd2-20, (sil\_score, low) }
    \label{fig:PCA}
\end{figure}




\section{Experimental- INTEL4}
\label{sec:experimental_result}
In this section, we describe our experiments on layout pattern generation as well as conduct analyses for its possible usage. 

\subsection{Experimental Setup}
\textbf{Dataset}: To evaluate our methodology
\textbf{Intel 4} dataset, we obtain the initial starter images by splitting a roughly 2000 x 2000 pixels initial layout into twenty 512 x 512 starter layout pattern images. Four tracks are picked from the initial layout and for each track, we crop into 5 starter images. This dataset only consists of 20 starter design rule clean images. The commercial tool is used to train the D
The purpose of this dataset is to validate our meth

\textbf{Diffusion model setting}: 
 We employed a family of pre-trained foundation models for image generation, specifically stablediffusion1.5-inpaint (PatternPaint) and stablediffusion2-inpaint (PatternPaint-ad) \cite{stablediffusion}. 

 
\textbf{Training details:} We adhered to the fine-tuning procedure described in DreamBooth \cite{ruiz2022dreambooth} to fine-tune the inpainting model with our data. The learning rate is set as 5e-6. All the starter clips, a total of 20, are used to fine-tune the model. Fine-tuning on PatternPaint and PatternPaint-ad models takes less than 10 mins on an NVIDIA A100 GPU. For PatternPaint, we denote its fine-tuned model as PatternPaint-finetune. For the PatternPaint-ad model, we denote its fine-tuned model as PatternPaint-finetune. We record the average processing time for each sample in our machine. One Nvidia A100 GPU is used for variation generations and one Intel(R) Xeon(R) Gold 6336Y CPU@2.40GHz is used for the legalization process. The average time for generating a sample was recorded at 0.81 seconds, and for legalizing a sample, it was 0.21 seconds.

%hotpot variate generation.

\input{PatPaint/tables/Intel4-Comparison}
Table~\ref{tab:comparison-Intel4} showcases our initial experiment using the twenty starter layout clips. We constrained mask selection to ten predefined types to more accurately assess model performance. Diversity metrics $H_1$ and $H_2$, calculated by the unique patterns, are also listed. For each combination of clip and mask, our model generated 100 variations, amounting to a total of 20,000 images. These images were subject to DR checks using the entire suite of DRs specified for the given layer. Across all four models, we observed the generation of 1000 to 2000 legal patterns.  There are a few replicated patterns, however, most of the patterns are unique and they enrich the current pattern library. Notably, there was an observed increase in both $H_1$ and $H_2$ for all models compared to the starter patterns.

The effectiveness of the proposed fine-tuning process is evident by comparing the PatternPaint model with PatternPaint-finetune, and PatternPaint-ad with PatternPaint-ad-finetune. It is seen by an increase in both the count of legal patterns and the number of unique patterns for the fine-tuned models. Diversity value, calculated using the aforementioned equation and legal patterns, shows that the fine-tuned PatternPaint-finetune model has the best performance. There is a significant increase in diversity compared to both the starter patterns and our model. However, an internally utilized heuristic-based pattern generation tool still surpassed all other methods. This superiority is attributed to the tool's manually encoded technology node and DR information, enabling efficient exploration within permissible ranges. The proposed model, on the other hand, relies on neighborhood information and random steps, and makes regional changes to 20 starter layout patterns, therefore, leading to a more clustered pattern library in the first round. In the later steps, however, we notice that more variations are produced through the iterative generation process.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/snap6_512.png}
    \caption{Starter Image}
    \end{subfigure} 
    \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/snap6_mask1_108_512.png}
    \caption{Generated Image 1}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/snap6_mask1_74_512.png}
    \caption{Generated Image 2}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/snap6_mask1_93_512.png}
    \caption{Generated Image 3}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/snap6_mask4_6_512.png}
    \caption{Generated Image 4}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{PatPaint/figs/snap6_mask4_104_512.png}
    \caption{Generated Image 5}
    \end{subfigure}
    \caption{Generated Variations from a single starter image}
    \label{fig:variations}
\end{figure}

Figure~\ref{fig:variations} visually represents the variations generated by the proposed methods. While the starter image is depicted in (a), (b-f) show the generated images. We notice that the proposed methods explored a wide range of variations, demonstrating models' awareness of tracks. For example, in (f), the model attempts to disconnect from an adjacent thick track and establish a connection with a farther one. In (e), more complex changes are made, forming connections with even farther tracks and upper objects.


\subsection{Iterative Pattern Generation}
Following the initial experiment, we created a library of unique patterns with substantial variation. We then embarked on iterative pattern generation, as per algorithms~\ref{alg:sample} and ~\ref{alg:iterativegeneration}, to check if diversity increased through this process. We designated the unique patterns from experiment 1 (Table 1) as our first iteration. For subsequent iterations, we conducted PCA analysis to select 100 of the most sparse representative samples, with the density constraint set at 40\% for the selected patterns. Using five predefined masks, we generated 5000 samples out of the 100 patterns, adding only clean and new samples to our existing pattern library.

Figure~\ref{fig:iterative} shows the experimental results as iterations increase. We evaluated four metrics: unique pattern count, image density, silhouette score, and entropy ($H_2$). Both unique pattern count and $H_2$ increased with each iteration. A notable gap was observed between baseline models (PatternPaint, PatternPaint-ad) and the fine-tuned models (PatternPaint-finetune, PatternPaint-ad-finetune), with the latter consistently outperforming the former. This further validates our fine-tuning process, demonstrating significant model improvements. Then, we examine the density of patterns in the current pattern library. This is because we observed that during iterative pattern generation, some models tend to take the easy path and produce sparse, empty areas in the masked region. While they are still legal and new patterns, these patterns are not useful. Therefore, we also keep track them during this process. For the starter images, the density is around 43.6\%. We noticed that only PatternPaint-ad-finetune matches the density in the starter layout clips. For all the other models, slight decreases are observed with PatternPaint and PatternPaint-finetune. For PatternPaint-ad, however, a higher density drop is observed, indicating that some sparse region exists in this existing pattern library. 

Lastly, we examine the silhouette score of our existing pattern library at each iteration. In order to obtain sil\_score, we first decrease the dimensionality of images using PCA. We use a large number of principal components to preserve 90\% of the explained variance in the dataset. Then we perform K-means clustering for these decomposed components. A number of 20 clusters are selected since we start from 20 distinct starter layout clips. An average sil\_score is computed for each iteration and shown in Figure~\ref{fig:iterative}. As iterations increase, we observe a constant decrease in sil\_score, indicating better diversity. PatternPaint-ad-finetune significantly outperforms other three models with lower sil\_score. This shows that PatternPaint-ad-finetune is able to produce more interesting variations than other models and the variations are not limited to the space around starter patterns. This also aligns with our observations in density analysis where PatternPaint-ad-finetune is able to produce high-density patterns that involve more risky changes.

Figure~\ref{fig:PCA} provides a 3D PCA plot interpretation of the silhouette scores. We selected the PatternPaint-finetune model (high silhouette score) and the PatternPaint-ad-finetune model (low silhouette score) for the PCA plots. The yellow points represent data from iteration 1, while the red points indicate data from iteration 7 in the pattern library. The PatternPaint-finetune plot shows more distinct clustering, whereas the PatternPaint-ad-finetune plot features less pronounced clusters and a denser distribution of samples across the region. This observation aligns with the silhouette scores, indicating the PatternPaint-ad-finetune model's superior performance in generating diverse patterns.

% add runtime if time permits added
\imprv{make runtime a table?}

\subsection{Analysis}
To further demonstrate the advantages of PatternPaint and its ability to take in DRC feedback as violated region, we present two application scenarios as case studies below.

\subsubsection{Case Study 1: Single Design Rule Correction}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\textwidth]{PatPaint/figs/Case1.pdf}
    \caption{DRV layout and fixed layouts}
    \label{fig:case1}
\end{figure}

Figure~\ref{fig:case1} details our experiment on a single Design Rule Violated (DRV) layout, where the DRC flagged a region (highlighted in red) due to incorrect width. We explored different masking options: Mask-0 used the original flagged region, Mask-1 expanded it by 25\%, and Mask-2 by 50\%. PatternPaint generated 20 variations for each mask, successfully exploring correct widths as shown in Figure 9(b). Notably, our model identified feasible widths from a limited set within 60 attempts. Figure~\ref{fig:case1} (c) shows another attempt to remove the connection between neighboring tracks that results in a DR Clean layout.

\subsubsection{Case Study 2: Multiple Design Rule Violations Correction}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\textwidth]{PatPaint/figs/Case2.pdf}
    \caption{Interesting patterns found after the Design Rule Corrections}
    \label{fig:case2}
\end{figure}

In our larger scale DRV correction experiment, we used violated layouts from the PatternPaint-ad-finetune iteration 2 as starter images, expanding the flagged regions by 25\% to construct masks. To prevent model performance degradation, we excluded masks exceeding 30\% of the image size, resulting in a total of 3863 starter images. Post-generation and DR Check, 57 patterns were deemed DR clean. Although a decrease in the percentage of legal patterns was observed compared to previous experiments, several intriguing patterns emerged, as depicted in Figure~\ref{fig:case2}. These included a new pattern on a different track (Figure~\ref{fig:case2}(a)) and a pattern with an unexplored width (Figure~\ref{fig:case2}(b)). In general, these variations are preferred by the foundry and it would be hard to observe by squish-based approach as it requires the addition of new squish lines. 


==> PatPaint/algs/Iterative_Generation.tex <==
% Until the Diversity target is reached and the sample budget is
% extended
% – From the existing pattern library, select patterns with high
% diversity score
% – Use PatPaint to create variations for these patterns using the predefined masks
% – Feed into design rule check to filter out illegal patterns

\begin{algorithm}
\caption{Iterative Generation}
\begin{algorithmic}[1]
\Require $X$ (starter layout patterns), $Sample\_budget$, $Score\_diversity$
\Ensure $diverse layout pattern library$ 

\While {Until diversity score or sample budget is reached}
\State Extract $n (n=100)$   most representative samples from existing library using PCA analysis
\State Perform Variations generation using Patpaint 
\State Perform DRC to filter out illegal solution and add new unique patterns to existing library

\State \Return $diverse layout pattern library$ 

\end{algorithmic}
\label{alg:iterativegeneration}
\end{algorithm}

==> PatPaint/tables/EUV-Comparison.tex <==
%\setlength{\tabcolsep}{5pt}

% \begin{table}[!tb]
% \caption{Quantitative Comparison on synthetic EUV 7nm dataset. A noise is defined as three of its surrounding pixels having the opposite values with the current pixel. Noise level counts the percentage of these noise pixels in an image. 
%  }
%  \label{tab:EUV_Comparison}
% \label{tab:comparison}
% \scriptsize
% \resizebox{\linewidth}{!}{
% %\begin{tabular}{|l|c|c|c|c|}
% \begin{tabular}{lccccc}
% %\toprule
% \hline
% \textbf{Method} & \textbf{\begin{tabular}[c]{@{}c@{}} Starter\\ Patterns\end{tabular}}  & 
% \textbf{\begin{tabular}[c]{@{}c@{}} Generated \\ Patterns\end{tabular}} &\textbf{\begin{tabular}[c]{@{}c@{}} Legal \\ Patterns\end{tabular}} & \textbf{Noise Level (\%) }\\ %\hline
% %\midrule
% \hline
%  CUP\cite{CUP}(VCAE) & 1000 & 2000 & 0& 8.76 \\ \\
%   CUP\cite{CUP}(VCAE+LegalGAN) & 1000 & 2000 & 0& 0.54 \\ \\
%  DiffPattern\cite{Diffpattern} & 20 & 2000 &  0 & 98.7  \\    \\   
%  DiffPattern\cite{Diffpattern} & 200 & 2000 & 13 & 4.02 \\ \\
%   DiffPattern\cite{Diffpattern} & 1000 & 2000 & 566 & 0.44\\ \\
%    PatternPaint\cite{Diffpattern}& 0 & 2000 & \textbf{820} & \textbf{0.03} \\
% \bottomrule
% \end{tabular}
% }
% %\vspace{-0.1in}
% \end{table}


% %ACM format
%\setlength{\tabcolsep}{5pt}

\begin{table}[!tb]
\caption{Quantitative comparison on synthetic EUV 7nm dataset. A noise is defined as three of its surrounding pixels having the opposite values with the current pixel. Noise level counts the percentage of these noise pixels in an image. 
 }
 \label{tab:EUV_Comparison}
\label{tab:comparison}
\scriptsize
\resizebox{\linewidth}{!}{
%\begin{tabular}{|l|c|c|c|c|}
\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \textbf{\begin{tabular}[c]{@{}c@{}} Starter\\ Patterns\end{tabular}}  & 
\textbf{\begin{tabular}[c]{@{}c@{}} Generated \\ Patterns\end{tabular}} &\textbf{\begin{tabular}[c]{@{}c@{}} Legal \\ Patterns\end{tabular}} & \textbf{Noise Level (\%) }\\ %\hline
\midrule
 CUP\cite{CUP}(VCAE) & 1000 & 2000 & 0& 8.76 \\ \\
  CUP\cite{CUP}(VCAE+LegalGAN) & 1000 & 2000 & 0& 0.54 \\ \\
 DiffPattern\cite{Diffpattern} & 20 & 2000 &  0 & 98.7  \\    \\   
 DiffPattern\cite{Diffpattern} & 200 & 2000 & 13 & 4.02 \\ \\
  DiffPattern\cite{Diffpattern} & 1000 & 2000 & 566 & 0.44\\ \\
   PatternPaint& 0 & 2000 & \textbf{820} & \textbf{0.03} \\
\bottomrule
\end{tabular}
}
%\vspace{-0.1in}
\end{table}

==> PatPaint/tables/Position_table.tex <==
%\setlength{\tabcolsep}{5pt}
% \begin{table}[!tb]
% \caption{Comparison for pre-trained models as well as internal tool performance
%  }
% \label{tab:comparison}
% \scriptsize
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \toprule
% %\hline
% & Heuristic solutions \cite{VIPER} & \\ DeePattern\cite{Deepattern} & VCAEwLegalGAN \cite{CUP} & LayouTransformer \cite{LayouTransformer} & DiffPattern\cite{Diffpattern} & Ours%\hline
% \midrule
%  Engineering effort & High & Medium & Low & Low & Medium
%  # of Training samples & None & 10k$\uparrow$ & 10k$\uparrow$ & 10k$\uparrow$ & 10k$\uparrow$ & 20 $\downarrow$
%  Technology-independent & No & No & No & No & No & Yes
% \bottomrule
% \end{tabular}
% %\vspace{-0.1in}
% \end{table}


\begin{table*}
    \centering
    \footnotesize
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
& Heuristic solutions \cite{VIPER,VTS} &  DeePattern\cite{Deepattern} & CUP \cite{CUP} & LayouTransformer \cite{LayouTransformer} & DiffPattern\cite{Diffpattern} & Ours \\ \hline \hline
ML Model Architecture & - & TCAE & VCAE & Transformer & Diffusion model & \begin{tabular}[c]{@{}c@{}}Pre-trained Diffusion model\\ with Inpainting \end{tabular} \\ \hline
Layout representation & - & squish & squish & Sequential Modeling & squish & pixel \\ \hline
 
 Engineering effort & High & Medium & \textbf{Low} & \textbf{Low} & Medium & \textbf{Low} \\  \hline
 \# of Training samples & None & 10k$\uparrow$ & 10k$\uparrow$ & 10k$\uparrow$ & 10k$\uparrow$ & \textbf{20 $\downarrow$} \\ \hline
 Technology-independent & No & No & No & No & No & \textbf{Yes} \\ \hline
    \end{tabular}}
    \caption{A Qualitative comparison with the existing works. }
    \label{tab:position-comparison}
\end{table*}
